Contract agreements via logic

We relate two contract models: one based on event structures and game theory, and the other one based on logic. In particular, we show that the notions of agreement and winning strategies in the game-theoretic model are related to that of provability in the logical model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{M. Carbone, I. Lanese, A. Lluch-Lafuente, A. Sokolova (Eds.):\\
6th Interaction and Concurrency Experience (ICE 2013)\\
EPTCS 131, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.131.2}{10.4204/EPTCS.131.2}}
\pdfoutput=1

